PACC: A Passive-Arm Approach for High-Payload Collaborative Carrying with Quadruped Robots Using Model Predictive Control

In this paper, we introduce the concept of using passive arm structures with intrinsic impedance for robot-robot and human-robot collaborative carrying with quadruped robots. The concept is meant for a leader-follower task and takes a minimalist approach that focuses on exploiting the robots' payload capabilities and reducing energy consumption, without compromising the robot locomotion capabilities. We introduce a preliminary arm mechanical design and describe how to use its joint displacements to guide the robot's motion. To control the robot's locomotion, we propose a decentralized Model Predictive Controller that incorporates an approximation of the arm dynamics and the estimation of the external forces from the collaborative carrying. We validate the overall system experimentally by performing both robot-robot and human-robot collaborative carrying on a stair-like obstacle and on rough terrain.

==> 04_controller_original.tex <==
\section{Locomotion Guidance and Control} \label{sec:locomotion}
In this section, we first describe how the velocity references
are generated using the passive arm for a robot that needs to act
as a follower. After that, we describe how the foot contacts are
planned and how the external forces at the end-effector are estimated, 
which are important elements of the proposed MPC formulation
presented at the end. 

\subsection{Locomotion Guidance} \label{sec:guidance}
To drive the robot in a collaborative carrying task where a leader
(another robot or a person) is in charge of choosing the path,
we propose a simple approach using the angular displacements of
the passive arm to generate motion references. In synthesis,
the \textit{follower-robot}, or just \textit{follower}, is commanded in terms of forward
velocity (velocity along the longitudinal axis of its horizontal
frame \cite{barasuol13icra}) and heading velocity. The desired
forward velocity and heading velocity are computed according to
the displacement of Joint 3 and Joint 1,
respectively, as illustrated in Fig. \ref{fig:arm_vel_commands}.
There, the green range represents the
neutral angular range where the desired velocity is zero. The
blue range refers to the first velocity level and the red range
the second level (with increased velocity). Since such velocity
modulation is discontinuous, we apply a second-order low-pass
filter to smooth out the command signals. The values for the range limits,
defined by $\theta$ and $\psi$, and the velocities considered in
this paper are detailed in Sec.
\ref{sec:results}.


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{images/victor/passive_arm/arm_vel_commands.pdf}
    \caption{Velocity command zones according to the arm joint displacements: on the left,
    lateral view showing the angular ranges used to obtain the desired robot forward velocity,
    where $\theta$ is the orientation of Joint 3 with respect to the gravity vector;
    on the right, top view showing the angular ranges used to obtain the desired robot's
    heading velocity, where $\psi$ is the angular position of Joint 1.}
    \label{fig:arm_vel_commands}
\end{figure}

\subsection{Foot Trajectory Generation}
Each foot performs a cubic spline between foot contact positions based on the gait parameters and on the desired $x$ (longitudinal) and $y$ (lateral) body velocities. Thus, the nominal $xy$ coordinates of the footholds of the $i$th leg at the horizontal frame are defined as 
\begin{equation}
    \label{eq:footholdnom_xy}
    {\FootPosNomXY}_i = {\FootPosCenterH} + \frac{1}{2}\frac{\dutygait}{\stepfreq}\UserVfxyH + {\deltaFootPA}_i
\end{equation}
where ${\FootPosCenter}_i$ is the foot default position (\textit{home position}), $\dutygait$ is the ratio of the stance period and the step period, $\stepfreq$ is the step frequency, $\UserVfxyH$ is the desired $xy$ velocity defined in the horizontal frame; and ${\deltaFootPA}_i$ is a correction term to adjust the support polygon due to external forces at the end-effector
\begin{equation}
    \label{eq:foothold_deltaforce}
    \deltaFootPA = 
    {
    % \renewcommand*{\arraystretch}{1.75}
    \Large
    \begin{bmatrix}
        \frac{\PAFeeHx\PAPeeHz - \PAFeeHz\PAPeeHx}{\massRobot\gravity - \PAFeeHz}&
        \frac{\PAFeeHy\PAPeeHz - \PAFeeHz\PAPeeHy}{\massRobot\gravity - \PAFeeHz}
    \end{bmatrix}}\Transp\text{,}
\end{equation}
where ${\PAFeeH}$, ${\PAPeeH}$ are the force and the position of the end-effector in the horizontal frame; $\massRobot$ is the total mass of the robot, and $\gravity$ is the gravity value.
%If ${\deltaFootPA}_x > 0$, the correction is applied only on the front legs;
%if ${\deltaFootPA}_x < 0$, then the correction is applied on the hind legs.
%Similarly, if ${\deltaFootPA}_y > 0$, the correction is applied only on the right legs,
%and if ${\deltaFootPA}_y < 0$, on the left legs.

The $\FootPosNomZ$ component of the foothold is computed based on the previous lift-off height $\FootPosLiftOffZ$, the desired linear velocity, and the desired angular rate $\CoMAngRateDesired$ of the robot's CoM
\begin{equation}
    \label{eq:footholdnom_z}
    %{\FootPosNomZI} = {\FootPosLiftOffZ}_i -  \frac{\dutygait}{\stepfreq}(\rotMatBTOH(\UserVf + \CoMAngRateDesired \times \FootPos_i))_z\text{,}
    {\FootPosNomZI} = {\FootPosLiftOffZ}_i -  \frac{\dutygait}{\stepfreq}
    \UserVz\text{,}
\end{equation}
where $\UserVz$ is the desired linear velocity for the base projected in the direction of the locally estimated terrain inclination. The next footholds in the world frame are predicted based on the desired velocity and remaining swing time of the $i$th leg ${\DeltaSwingtime}_i$
\begin{equation}
    \label{eq:footholdnom}
    {\FootPosNom}_i = \rotMatHTOW{\FootPosNomHI} + \CoMposlin + {\DeltaSwingtime}_i\rotMatHTOW\UserVf\text{,}
\end{equation}
where $\rotMatHTOW$ is the rotation from horizontal to world frame, ${\FootPosNomHI}$ is the nominal foothold with components defined by \eqref{eq:footholdnom_xy} and \eqref{eq:footholdnom_z}; and $\CoMposlin \in \Real^3$ is the position of the robot's CoM in the world frame.


\subsection{Locomotion Controller} \label{sec:controller}

\subsubsection{End-effector Force Estimation}
Let us consider the dynamic model of the passive arm subject to an external force in the end-effector
\begin{equation}
    \label{eq:passive_arm_model}
    \PAinertiaM\PAjointAcc + \PAV = \PAtauG + \PAtauSpring + \PAtauDamper + \PAJee\Transp\PAFee\text{,}
\end{equation}
where $\PAjoint \in \Real^3$ is the joint position of the passive arm, $\PAinertiaM \in \Real^{3\times3}$ is the inertia matrix, $\PAV \in \Real^3$ captures the Coriolis effect, $\PAtauG \in \Real^3$ is the gravitational torque, $\PAtauSpring \in \Real^3$ is the torque from the joint stiffness,
$\PAtauDamper \in \Real^3$ is the torque from the joint damping, $\PAJee \in \Real^{3\times3}$ is the end-effector Jacobian, and $\PAFee \in \Real^3$ is the force applied at the end-effector. Due to the low inertia of the third link, and assuming small joint velocities and small accelerations for the first and second joints, the terms $\PAinertiaM\PAjointAcc$ and $\PAV$ can be neglected. Hence, the force is computed as
\begin{equation}
    \label{eq:est_ext_force_ee}
    \KFFeeEst = -(\PAJee\Transp)^{-1}(\PAtauG + \PAtauSpring + \PAtauDamper) \text{,}
    %\PAFee = -(\PAJee\Transp)^{-1}(\PAtauG + \PAtauSpring + \PAtauDamper) \text{,}
\end{equation}
where $\PAtauSpring$ and $\PAtauDamper$ are computed as
\begin{equation}
    \PAtauSpring = -\PASpringCoef (\PAjoint - {\PAjoint}_0)\text{ and }\PAtauDamper = -\PADamperCoef \dot{\PAjoint} \text{,}
\end{equation}
where $\PASpringCoef$ and $\PADamperCoef$ are, respectively, the diagonal
matrices of spring and damping coefficients from Tab. \ref{tab:joint_impedances},
and ${\PAjoint}_0$ is the vector of joint positions at the springs' equilibrium length. 

Thus, the equivalent force and torque in the robot's CoM described in the world frame are
\begin{gather}
    \label{eq:force_torque_ext}
    \begin{aligned}
        \ForceExt &= \rotMatBTOW\KFFeeEst\text{,}&
        \TorqueExt &= \rotMatBTOW \PAPee^B \times \KFFeeEst\text{,}
    \end{aligned}
\end{gather}
%where $\rotMatBTOW$ is the rotation matrix between world and base frames, and 
where $\PAPee^B$ is the end-effector position in the base frame.



\subsubsection{MPC}
A nonlinear MPC is formulated to compute ground reaction forces (GRFs) and foot positions to track a desired CoM's trajectory.  Similar to \cite{nmpc_angelo}, a
Single Rigid Body Dynamics (SRBD) model is considered
\begin{gather}
    \label{eq:srbd_model}
    \begin{aligned}
    &\massRobot(\ddot{\CoMposlin} - \gravityArray) = \sum_{i=1}^4 \contactFlag_i\Grf_i + \ForceExt\text{, }\ \ \
    %
    \dot{\CoMposang} =  \TransOmegaToEuler(\CoMposang)\CoMvelang\text{,}
    \\
    %
    &\inertiaRobot\dotCoMvelang + \CoMvelang\times \inertiaRobot{\CoMvelang}  = \sum_{i=1}^4 \contactFlag_i\contactPoint_i \times \rotMatBTOW\Grf_i + \rotMatBTOW\TorqueExt\text{,}\\
    %
    % \dot{\CoMposang} &=  \TransOmegaToEuler(\CoMposang)\CoMvelang\text{,}
    \end{aligned}
\end{gather}
omitting the swing legs' dynamics. In \eqref{eq:srbd_model},  $\CoMposlin \in \Real^3$ is the position of the CoM in the world frame, $\gravityArray \in \Real^3$ is the gravity vector; $\inertiaRobot^{3\times3}$ is the inertia tensor of the robot given in the base frame; $\contactPoint_i \in \Real^3$ is the $i$th foot position given in the base frame; $\Grf_i \in \Real^3$ is the GRF of the $i$th foot, and $\contactFlag_i$ is the contact state variable of the $i$th foot; $\TransOmegaToEuler(\CoMposang) \in \Real^{3\times3}$ is the transformation matrix between the angular velocity $\CoMvelang\in \Real^3$ in the base frame and the rate of the Euler angles $\dot{\CoMposang}$; $\ForceExt$ and $\TorqueExt$ are external forces and torques applied in the CoM. In order to optimize the footholds location $\contactPoint_i$, we augment the input space of the controller by an additional variable $\FootVelOpt \in \Real^{12}$, obtaining a simplified model for the $i$th foot position dynamics as 
\begin{equation}
    \label{eq:foot_model}
    \FootVel_i = (1 - \contactFlag_i) \FootVelOpt_i\text{.}
\end{equation}



%Considering as external disturbances only forces acting at the end-effector
%of the passive arm, i.e., $\dss = \begin{bmatrix}\ForceExt\Transp &
%\TorqueExt\Transp\end{bmatrix}\Transp$, the displacement between the robot's
%CoM and the end-effector represents a disturbance. Considering the end-effector
%does not move and the components ${\mathrm{f}_\mathrm{ext}}_z$,
%${\tau_\mathrm{ext}}_\phi$, ${\tau_\mathrm{ext}}_\theta$ are negligible,
%the prediction of the disturbance is obtained based on the equivalent cartesian
%impedance
Considering as external disturbances only the forces acting at the end-effector and that
they can be estimated using Eq. \ref{eq:est_ext_force_ee} and Eq. \ref{eq:force_torque_ext},
it is possible to include in the prediction model an approximation for the evolution of such forces
due to the movement of the base. To do so, we simplify the modeling assuming that both the
end-effector and the base can move independently from each other and that the end-effector
positions along the horizon are known. This way, the distance between them along the horizon is given 
by:
\begin{equation}
\Delta_{er} = \PAPee^0 - \CoMposlin
\end{equation}
where $\PAPee^0$ is the end-effector known position along the horizon. If all forces between
the end-effector and the base are assumed only caused by the deformation of the springs, the
disturbance and its evolution are given as:
%of the forces 
%end-effector can be  
%i.e., $\dss = \begin{bmatrix}\ForceExt\Transp & \TorqueExt\Transp\end{bmatrix}\Transp$, here we introduce the the displacement between the robot's %CoM and the end-effector represents a disturbance. Considering the end-effector does not move and the components ${\mathrm{f}_\mathrm{ext}}_z$, %${\tau_\mathrm{ext}}_\phi$, ${\tau_\mathrm{ext}}_\theta$ are negligible, the prediction of the disturbance is obtained based on the equivalent %cartesian impedance
%
\begin{equation}
    \dss = \begin{bmatrix}
        \mathrm{f}_{\mathrm{ext}_x} - \BarPASpringCoefScalar{}_x \Delta^0_{{er}_x} \\
        \mathrm{f}_{\mathrm{ext}_y} - \BarPASpringCoefScalar{}_y \Delta^0_{{er}_y} \\
        0\\
        0\\
        0\\
        \tau_{{\mathrm{ext}}_z} - ||\Delta_{er}||^2\BarPASpringCoefScalar{}_y (\psi^0 - \psi)
    \end{bmatrix}
\end{equation}
\begin{equation}
    \label{eq:ext_disturbance_model}
    \dot{\dss} = \begin{bmatrix}
        -\BarPASpringCoefScalar{}_x \CoMvellinx&
        -\BarPASpringCoefScalar{}_y \CoMvelliny&
        0&
        0&
        0&
        -||\Delta_{er}||^2\BarPASpringCoefScalar{}_y\YawVel
    \end{bmatrix}
\end{equation}
where
\begin{gather}
\begin{aligned}
    \label{eq:fext_passive_arm}
    &\BarPASpringCoef = (\PAJee\Transp\rotMatWTOB)^{-1}\PASpringCoef(\rotMatBTOW\PAJee)^{-1} = 
    \mathrm{diag}(\BarPASpringCoefScalar{}_x,\BarPASpringCoefScalar{}_y,\BarPASpringCoefScalar{}_z)
\end{aligned}
\end{gather}


For ensuring dynamic stability, the ZMP is constrained to be inside the support polygon, e.g. the convex-hull generated by the leg of the robot in stance, which is defined based on the momentum associated with the passive arm end-effector~\cite{handbook_legged} as
\begin{gather}
    \label{eq:zmp_def}
    \begin{aligned}
        \xZMP = \frac{\massRobot\gravity \CoMposlinx - \CoMposlinz \massRobot\ddot{\CoMposlinScalar}_x - \PAPeex\PAFextz + \PAPeez\PAFextx}{\massRobot\gravity - \PAFextz}\text{,}\\
        \yZMP = \frac{\massRobot\gravity \CoMposliny - \CoMposlinz \massRobot\ddot{\CoMposlinScalar}_y - \PAPeey\PAFextz + \PAPeez\PAFexty}{\massRobot\gravity - \PAFextz}\text{,}
    \end{aligned}
\end{gather}
where $\CoMposlinScalar_j$, ${\PAPeeScalar}_j$, ${\PAFextScalar}_j$ are the components of $\CoMposlin$, $\PAPee$, and $\ForceExt$, respectively, with $j \in \{ x,y,z\}$. 

%To track a desired CoM's linear and angular trajectories, 
Finally, the state, control, and disturbance vector are defined as
\begin{gather}
    \label{eq:x_u_d_def}
    \begin{aligned}
    \xss &=
    \begin{bmatrix}
        \CoMposang\Transp &
        \CoMposlin\Transp &
        {\CoMvelang}\Transp &
        \dot{\CoMposlin}\Transp &
        \FootPos\Transp &
        \dss\Transp
    \end{bmatrix}\Transp\text{,}\\ 
    \uss &=
    \begin{bmatrix}
        \Grf\Transp & \FootVelOpt\Transp
    \end{bmatrix}\Transp\text{, }
    % \dss =
    % \begin{bmatrix}
    %     \ForceExt\Transp & \TorqueExt\Transp
    % \end{bmatrix}\Transp\text{,}
\end{aligned}
\end{gather}
%where $\xss \in \Real^{24}$, $\uss \in \Real^{24}$, $\dss \in \Real^6$.
with $\xss \in \Real^{30}$ and $\uss \in \Real^{24}$. 

Given a periodic contact sequence that defines $\contactFlag$ along the prediction horizon $\Ny$, an optimization problem is formulated to track a desired state trajectory $\xref$
\begin{align}
    \label{eq:opt_mpc}
    &\underset{\Xopt_k,\Uopt_k}{\text{min}} &&
    \sum_{i=0}^{\Ny}\|{\xref}{}_{k+i} - \xss{}_{k+i}\|^2_{\Qfc}  + \sum_{i=0}^{\Ny-1}\|\uss{}_{k+i}\|^2_{\Rfc} + \|\boldsymbol{\epsilon}_{k+i}\|^2_\rho \\
    &\textit{s.t.}&& \xss_k = \xss_0\text{,}
    \\&&&
    \label{eq:model_function}
    \xss_{k+i+1} = \boldsymbol{g}(\xss{}_{k+i},\uss{}_{k+i},\contactFlagVector{}_{k+i})\text{,}
    \\&&&
    \label{eq:fc_contraint}
    \hFriction(\uss{}_{k+i}) \leq \ZeroMat\text{,}
    \\&&&
    \label{eq:zmp_contraint}
    \hZmp(\xss{}_{k+i}, \uss{}_{k+i}) + \boldsymbol{\epsilon}_{k+i} \leq \ZeroMat\text{,}
\end{align}
where $\Xopt_k$ and $\Uopt_k$ are the state and control actions along $\Ny$; $\xss_0$ is the current state using the values of $\ForceExt$ and $\TorqueExt$ given by \eqref{eq:force_torque_ext}; \eqref{eq:model_function} is the prediction model defined by \eqref{eq:srbd_model}, \eqref{eq:foot_model}, and \eqref{eq:ext_disturbance_model}; \eqref{eq:fc_contraint} comprehends the friction constraint defined by a pyramidal approximation and maximum force constraint~\cite{nmpc_angelo}; \eqref{eq:zmp_contraint} constrains the ZMP \eqref{eq:zmp_def} to be inside the support polygon defined by the leg in stance at time $k+i$, and $\boldsymbol{\epsilon}$ is an additional slack variables employed to avoid a potential infeasibility of the MPC. These variables, in fact, permit a small violations of the ZMP constraints instead of incurring in a failure of the MPC solver, and are heavily penalized in \eqref{eq:opt_mpc} by using the weight $\rho$. Finally, $\Qfc$, $\Rfc$, are diagonal weighting matrices that define the importance of the tracking error for each robot's state and input. 

The MPC\footnote{https://github.com/iit-DLSLab/Quadruped-PyMPC/} has been implemented using Acados~\cite{acados}, an open-source Sequential Quadratic Programming solver tailored for optimal control, employing HPIPM~\cite{HPIPM} as a quadratic solver. 
% \begin{table}[h]
% \centering
% \begin{tabular}{ccc}
% \toprule
% \textbf{Parameter} & \textbf{Value} & \textbf{Unit}
% \midrule
% \massRobot & d & Kg
% \Ny & d & -\\
% \bottomrule
% \end{tabular}
% \caption{PACC linear and angular kinematic parameters.}
% \label{tab:parameters}
% \end{table}


%%%%%%%%%%%%%%%% SMPC %%%%%%%%%%%%%%%%
\iffalse % Removing since we will not use it :( 
\subsubsection{Stochastic MPC (SMPC) \textcolor{red}{(include if it works)}}
The system representation given by \eqref{eq:model_function} can be denominated deterministic and \textit{nominal}. A general form to consider additive uncertainties is
\begin{equation}
    \label{eq:model_smpc}
    \xss_{k+1} = \ModelFunction(\xss{}_{k},\uss{}_{k},\dss{}_{k},\contactFlagVector{}_{k}) + \Dss\wss{}_{k}\text{,}
\end{equation}
where $\wss{}_k \in \Real^3$ is assumed independent and identically distributed (i.i.d.) with a known probability distribution, e.g., as a Gaussian distribution, i.e., $\wss \thicksim \normalDist(0, \Sigma^\wss)$; and $\Dss$ maps the states affected by $\wss{}_k$.

Due to the estimation of the external forces and torques, the system's uncertainties are related to the evolution of $\dot{\CoMposlin}$ and $\CoMvelang$, resulting in the following mapping matrix $\Dss$ \textcolor{red}{(to be updated)}
\begin{equation}
    \Dss = \begin{bmatrix}
        \EyeTr & \ZeroMat_{3\times3} & \EyeTr & \ZeroMat_{3\times3}
    \end{bmatrix}\Transp\text{.}
\end{equation}


Due to the presence of uncertainty in the system model, it is necessary to include a tightened term $\CClambda$ into the ZMP constraint to compensate for the influence of $\wss_k$. Thus, the constraint~\eqref{eq:zmp_contraint} is reformulated as 
\begin{equation}
    \label{eq:zmp_constraint_with_lambda}
    \CZmp\xss{}_{k+1} \leq \hZmp - \CClambda{}_{k+1}\text{.}
\end{equation}


In robust strategies, e.g., RMPC, the tightened term $\CClambda{}$ can be computed based on the worst-case~\cite{kouvaritakis_cannon_book_2016}
\begin{equation}
    \label{eq:contraint_lambda_rmpc}
    {\CClambda{}_k}_j  = \max_{\wss_k\ \in\ \NoisePolytope}(\CBarZmp \Sw)_j \wss_{k}\text{,}
\end{equation}
where $\CBarZmp$ is the diagonal composition of $\Ny$ matrix $\CZmp$, i.e., $\CBarZmp= \mathrm{diag}(\CZmp,\dots,\CZmp)$; $\Sw$ defines the propagation of $\wss_k$ into the states along the prediction horizon; $\NoisePolytope = \{\wss: |\wss| \leq \wss_{\maxValue}\}$; and the subscript $j$ denotes the $j$th row of a matrix. However, this strategy is naturally conservative. The worst-case may never occur and operating close to the constraints usually results in a lower value of the cost function.

Considering the uncertainty as a random variable with probabilistic properties, SMPC reformulates the constraint~\eqref{eq:zmp_contraint} as a chance-constraint, yielding to
\begin{equation}
    \label{eq:chance_constraint_definition}
    \probCondition\{ \CZmp\xss{}_{k+1} \leq \hZmp \} \geq 1 - \probLevel\text{,}
\end{equation}
where $\probCondition\{ \mathcal{X} \}$ denotes the probability of the event $\mathcal{X}$ occurring, and $\probLevel$ is the maximum acceptable probability level of the constraint to be violated. For $\wss_k$ characterized as an unbounded signal with Gaussian Distribution, $\Expected[\wss_k] = 0$ and variance matrix $\NoiseVariance$, each $j$th row of $\CClambda_k$ in \eqref{eq:zmp_constraint_with_lambda} can be exactly computed as %
\begin{equation}
    \label{eq:lambda_gaussian_zmp_constraint}
    {\CClambda{}_k}_j(1-\probLevel) = (\CBarZmp \Sw)_{j}\Bar{\NoiseVariance}(\CBarZmp \Sw)_{j}^{\Transp}%\sqrt{(\CBarZmp \Sw)_{j}\Bar{\NoiseVariance}(\CBarZmp \Sw)_{j}^{\Transp}
    %}\CDF^\ScriptInv(1-\probLevel)\text{,}
\end{equation}
where $\Bar{\NoiseVariance}$ is the diagonal composition of $\Ny$ matrices $\NoiseVariance$, i.e., $\Bar{\NoiseVariance} = \mathrm{diag}(\NoiseVariance,\dots,\NoiseVariance)$; and $\CDF$ is the cumulative distribution function of a Gaussian variable with zero mean and unitary variance \cite{chance_constraints_path,convex_boyd}. As \eqref{eq:model_function} is linearized at each control step, and consequently, modifying $\Sw$ matrix, $\CClambda$ needs to be recomputed at each control step.

To consider the presence of uncertainty and the tightened term $\CClambda$ given by \eqref{eq:lambda_gaussian_zmp_constraint}, the optimization~\eqref{eq:opt_mpc} is redefined as
\begin{gather}
    \label{eq:opt_smpc}
    \begin{aligned}
    &\underset{\Xopt_k,\Uopt_k}{\text{min}} && 
    \Expected\Bigg[\sum_{i=0}^{\Ny}\|{\xref}{}_{k+i} - \xss{}_{k+i}\|^2_\Qfc  + \sum_{i=0}^{\Ny-1}\|\uss{}_{k+i}\|^2_\Rfc\Bigg]\\
    &\textit{s.t.}&& \xss_k = \xss_0\text{,}
    \\&&&
    \xss_{k+i+1} = \ModelFunction(\xss{}_{k+i},\uss{}_{k+i},\dss{}_{k+i},\contactFlagVector{}_{k+i})\text{,}
    \\&&&
    \KfConeFull\uss{}_{k+i} \leq \fcConeFull\text{,}
    \\&&&
    \CZmp\xss{}_{k+i} \leq \hZmp - \CClambda{}_{k+i}\text{.}
\end{aligned}
\end{gather}
\fi

==> 07_TODO.tex <==
\section{TO-DO LIST}
\begin{itemize}
    \item Collect references of robots that have the load attachment on top of the torso and insert them in Sec II.
\end{itemize}
